Does Terrorism Trigger Online Hate Speech? On the Association of Events and Time Series

Hate speech is ubiquitous on the Web. Recently, the offline causes that contribute to online hate speech have received increasing attention. A recurring question is whether the occurrence of extreme events offline systematically triggers bursts of hate speech online, indicated by peaks in the volume of hateful social media posts. Formally, this question translates into measuring the association between a sparse event series and a time series. We propose a novel statistical methodology to measure, test and visualize the systematic association between rare events and peaks in a time series. In contrast to previous methods for causal inference or independence tests on time series, our approach focuses only on the timing of events and peaks, and no other distributional characteristics. We follow the framework of event coincidence analysis (ECA) that was originally developed to correlate point processes. We formulate a discrete-time variant of ECA and derive all required distributions to enable analyses of peaks in time series, with a special focus on serial dependencies and peaks over multiple thresholds. The analysis gives rise to a novel visualization of the association via quantile-trigger rate plots. We demonstrate the utility of our approach by analyzing whether Islamist terrorist attacks in Western Europe and North America systematically trigger bursts of hate speech and counter-hate speech on Twitter.

==> ms-gnuplottex-fig1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter{}
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7160.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(737,2654){\makebox(0,0)[l]{\strut{}\scriptsize{\texttt{\#stopislam}}}}%
      \csname LTb\endcsname%%
      \put(257,1829){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1350,1829){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2455,1829){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3549,1829){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4660,1829){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5748,1829){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6853,1829){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(737,1790){\makebox(0,0)[l]{\strut{}\scriptsize{\texttt{\#notinmyname}}}}%
      \csname LTb\endcsname%%
      \put(257,966){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1350,966){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2455,966){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3549,966){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4660,966){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5748,966){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6853,966){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(737,927){\makebox(0,0)[l]{\strut{}\scriptsize{\texttt{kafir}}}}%
      \csname LTb\endcsname%%
      \put(257,102){\makebox(0,0){\strut{}\tiny{2015-01}}}%
      \csname LTb\endcsname%%
      \put(1350,102){\makebox(0,0){\strut{}\tiny{2015-07}}}%
      \csname LTb\endcsname%%
      \put(2455,102){\makebox(0,0){\strut{}\tiny{2016-01}}}%
      \csname LTb\endcsname%%
      \put(3549,102){\makebox(0,0){\strut{}\tiny{2016-07}}}%
      \csname LTb\endcsname%%
      \put(4660,102){\makebox(0,0){\strut{}\tiny{2017-01}}}%
      \csname LTb\endcsname%%
      \put(5748,102){\makebox(0,0){\strut{}\tiny{2017-07}}}%
      \csname LTb\endcsname%%
      \put(6853,102){\makebox(0,0){\strut{}\tiny{2018-01}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter{}
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7160.00,1720.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(23,17){\makebox(0,0)[l]{\strut{}\tiny{time}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(483,1492){\makebox(0,0)[l]{\strut{}\tiny{without serial dependencies}}}%
      \csname LTb\endcsname%%
      \put(55,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(164,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(272,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(381,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(490,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(598,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(707,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(815,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(924,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1032,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1141,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1250,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1358,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1467,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1575,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1684,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1792,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1901,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2010,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2118,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2227,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2335,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2444,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2552,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2661,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2770,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2878,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2987,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3095,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3204,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3312,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3421,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3530,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3638,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3747,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3855,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3964,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4072,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4181,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4289,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4398,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4507,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4615,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4724,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4832,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4941,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5049,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5158,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5267,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5375,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5484,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5592,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5701,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5809,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5918,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6027,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6135,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6244,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6352,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6461,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6569,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6678,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6787,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6895,760){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(7004,760){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(483,718){\makebox(0,0)[l]{\strut{}\tiny{with serial dependencies}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter{}
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4800.00,1440.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(612,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(751,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(890,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1030,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1169,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1308,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1447,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1586,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1726,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1865,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2004,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2143,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2282,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2422,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2561,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2700,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2839,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2978,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3118,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3257,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3396,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3535,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3674,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3814,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3953,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4092,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4231,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4370,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4510,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4649,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4788,821){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(480,432){\makebox(0,0)[r]{\strut{}\tiny{trigger}}}%
      \csname LTb\endcsname%%
      \put(480,302){\makebox(0,0)[r]{\strut{}\tiny{precursor}}}%
      \csname LTb\endcsname%%
      \put(640,43){\makebox(0,0)[l]{\strut{}\tiny{time}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(408,1223){\makebox(0,0){\strut{}$\mathcal{B}$ }}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(612,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(751,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(890,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1030,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1169,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1308,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1447,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1586,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1726,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1865,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2004,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2143,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2282,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2422,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2561,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2700,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2839,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2978,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3118,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3257,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3396,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3535,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3674,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3814,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3953,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4092,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4231,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4370,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4510,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4649,332){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4788,332){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(408,733){\makebox(0,0){\strut{}$\mathcal{A}$ }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter{}
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7160.00,3600.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1865,2012){\makebox(0,0)[l]{\strut{}$(\ast)$}}%
      \csname LTb\endcsname%%
      \put(2734,1494){\makebox(0,0)[l]{\strut{}$(\dagger)$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(175,1439){\makebox(0,0){\strut{}\small{$K_\text{tr}$}}}%
      \csname LTb\endcsname%%
      \put(2004,75){\makebox(0,0){\strut{}\small{threshold $\tau_m$}}}%
      \csname LTb\endcsname%%
      \put(685,567){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(685,785){\makebox(0,0)[r]{\strut{}\tiny{4}}}%
      \csname LTb\endcsname%%
      \put(685,1003){\makebox(0,0)[r]{\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(685,1221){\makebox(0,0)[r]{\strut{}\tiny{12}}}%
      \csname LTb\endcsname%%
      \put(685,1440){\makebox(0,0)[r]{\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(685,1658){\makebox(0,0)[r]{\strut{}\tiny{20}}}%
      \csname LTb\endcsname%%
      \put(685,1876){\makebox(0,0)[r]{\strut{}\tiny{24}}}%
      \csname LTb\endcsname%%
      \put(685,2094){\makebox(0,0)[r]{\strut{}\tiny{28}}}%
      \csname LTb\endcsname%%
      \put(685,2312){\makebox(0,0)[r]{\strut{}\tiny{32}}}%
      \csname LTb\endcsname%%
      \put(787,354){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(1135,354){\makebox(0,0){\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(1482,354){\makebox(0,0){\strut{}\tiny{2}}}%
      \csname LTb\endcsname%%
      \put(1830,354){\makebox(0,0){\strut{}\tiny{3}}}%
      \csname LTb\endcsname%%
      \put(2178,354){\makebox(0,0){\strut{}\tiny{4}}}%
      \csname LTb\endcsname%%
      \put(2526,354){\makebox(0,0){\strut{}\tiny{5}}}%
      \csname LTb\endcsname%%
      \put(2873,354){\makebox(0,0){\strut{}\tiny{6}}}%
      \csname LTb\endcsname%%
      \put(3221,354){\makebox(0,0){\strut{}\tiny{7}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3970,1439){\makebox(0,0){\strut{}\small{$r_\text{tr}$}}}%
      \csname LTb\endcsname%%
      \put(5798,75){\makebox(0,0){\strut{}\small{$p$-quantile}}}%
      \csname LTb\endcsname%%
      \put(5166,893){\makebox(0,0)[l]{\strut{}\small{independent}}}%
      \csname LTb\endcsname%%
      \put(5166,707){\makebox(0,0)[l]{\strut{}\small{dependent}}}%
      \csname LTb\endcsname%%
      \put(4480,540){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(4480,896){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(4480,1252){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(4480,1609){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(4480,1965){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(4480,2321){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(4582,354){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(5069,354){\makebox(0,0){\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(5555,354){\makebox(0,0){\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(6042,354){\makebox(0,0){\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(6528,354){\makebox(0,0){\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(7015,354){\makebox(0,0){\strut{}\tiny{1}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter{}
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7160.00,2300.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(714,595){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(714,824){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(714,1053){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(714,1283){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(714,1512){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(714,1741){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(816,409){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(1069,409){\makebox(0,0){\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(1322,409){\makebox(0,0){\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(1574,409){\makebox(0,0){\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(1827,409){\makebox(0,0){\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(2080,409){\makebox(0,0){\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(184,1168){\makebox(0,0)[l]{\strut{}$r_\text{tr}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(306,1168){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1448,130){\makebox(0,0){\strut{}$p$-quantile}}%
      \csname LTb\endcsname%%
      \put(1448,2020){\makebox(0,0){\strut{}MA order 0 (iid)}}%
      \csname LTb\endcsname%%
      \put(1322,1168){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{$\Delta=0$}}}}%
      \csname LTb\endcsname%%
      \put(2080,1913){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{$\Delta=64$}}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(3100,595){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(3100,824){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(3100,1053){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(3100,1283){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(3100,1512){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(3100,1741){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(3202,409){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(3455,409){\makebox(0,0){\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(3708,409){\makebox(0,0){\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(3960,409){\makebox(0,0){\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(4213,409){\makebox(0,0){\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(4466,409){\makebox(0,0){\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(2570,1168){\makebox(0,0)[l]{\strut{}$r_\text{tr}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2692,1168){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3834,130){\makebox(0,0){\strut{}$p$-quantile}}%
      \csname LTb\endcsname%%
      \put(3834,2020){\makebox(0,0){\strut{}MA order 32}}%
      \csname LTb\endcsname%%
      \put(3708,1168){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{$\Delta=0$}}}}%
      \csname LTb\endcsname%%
      \put(4125,1684){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{$\Delta=64$}}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(5487,595){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(5487,824){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(5487,1053){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(5487,1283){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(5487,1512){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(5487,1741){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(5589,409){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(5842,409){\makebox(0,0){\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(6095,409){\makebox(0,0){\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(6347,409){\makebox(0,0){\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(6600,409){\makebox(0,0){\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(6853,409){\makebox(0,0){\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(4957,1168){\makebox(0,0)[l]{\strut{}$r_\text{tr}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(5079,1168){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6221,130){\makebox(0,0){\strut{}$p$-quantile}}%
      \csname LTb\endcsname%%
      \put(6221,2020){\makebox(0,0){\strut{}MA order 128}}%
      \csname LTb\endcsname%%
      \put(6095,1168){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{$\Delta=0$}}}}%
      \csname LTb\endcsname%%
      \put(6423,1535){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{$\Delta=64$}}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig5}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig6.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter{}
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,10080.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(306,8418){\makebox(0,0){\strut{}$r_\text{tr}$}}%
      \csname LTb\endcsname%%
      \put(2465,6850){\makebox(0,0){\strut{}$p$-quantile}}%
      \csname LTb\endcsname%%
      \put(2465,9800){\makebox(0,0){\strut{}\texttt{\#stopislam} ($\hat{p}=.0317$)}}%
      \csname LTb\endcsname%%
      \put(1400,7969){\makebox(0,0)[l]{\strut{}\scriptsize{95\% }}}%
      \csname LTb\endcsname%%
      \put(1400,7737){\makebox(0,0)[l]{\strut{}\scriptsize{expected}}}%
      \csname LTb\endcsname%%
      \put(1400,7505){\makebox(0,0)[l]{\strut{}\scriptsize{observed}}}%
      \csname LTb\endcsname%%
      \put(714,7315){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(714,7756){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%%
      \put(714,8197){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%%
      \put(714,8639){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%%
      \put(714,9080){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%%
      \put(714,9521){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(816,7129){\makebox(0,0){\strut{}$0.75$}}%
      \csname LTb\endcsname%%
      \put(1476,7129){\makebox(0,0){\strut{}$0.8$}}%
      \csname LTb\endcsname%%
      \put(2136,7129){\makebox(0,0){\strut{}$0.85$}}%
      \csname LTb\endcsname%%
      \put(2795,7129){\makebox(0,0){\strut{}$0.9$}}%
      \csname LTb\endcsname%%
      \put(3455,7129){\makebox(0,0){\strut{}$0.95$}}%
      \csname LTb\endcsname%%
      \put(4115,7129){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(306,5058){\makebox(0,0){\strut{}$r_\text{tr}$}}%
      \csname LTb\endcsname%%
      \put(2465,3490){\makebox(0,0){\strut{}$p$-quantile}}%
      \csname LTb\endcsname%%
      \put(2465,6440){\makebox(0,0){\strut{}\texttt{\#notinmyname} ($\hat{p}=.2075$)}}%
      \csname LTb\endcsname%%
      \put(1400,4609){\makebox(0,0)[l]{\strut{}\scriptsize{95\%}}}%
      \csname LTb\endcsname%%
      \put(1400,4377){\makebox(0,0)[l]{\strut{}\scriptsize{expected}}}%
      \csname LTb\endcsname%%
      \put(1400,4145){\makebox(0,0)[l]{\strut{}\scriptsize{observed}}}%
      \csname LTb\endcsname%%
      \put(714,3955){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(714,4396){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%%
      \put(714,4837){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%%
      \put(714,5279){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%%
      \put(714,5720){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%%
      \put(714,6161){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(816,3769){\makebox(0,0){\strut{}$0.75$}}%
      \csname LTb\endcsname%%
      \put(1476,3769){\makebox(0,0){\strut{}$0.8$}}%
      \csname LTb\endcsname%%
      \put(2136,3769){\makebox(0,0){\strut{}$0.85$}}%
      \csname LTb\endcsname%%
      \put(2795,3769){\makebox(0,0){\strut{}$0.9$}}%
      \csname LTb\endcsname%%
      \put(3455,3769){\makebox(0,0){\strut{}$0.95$}}%
      \csname LTb\endcsname%%
      \put(4115,3769){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(306,1698){\makebox(0,0){\strut{}$r_\text{tr}$}}%
      \csname LTb\endcsname%%
      \put(2465,130){\makebox(0,0){\strut{}$p$-quantile}}%
      \csname LTb\endcsname%%
      \put(2465,3081){\makebox(0,0){\strut{}\texttt{kafir} ($\hat{p}=.3561$)}}%
      \csname LTb\endcsname%%
      \put(1400,1249){\makebox(0,0)[l]{\strut{}\scriptsize{95\%}}}%
      \csname LTb\endcsname%%
      \put(1400,1017){\makebox(0,0)[l]{\strut{}\scriptsize{expected}}}%
      \csname LTb\endcsname%%
      \put(1400,785){\makebox(0,0)[l]{\strut{}\scriptsize{observed}}}%
      \csname LTb\endcsname%%
      \put(714,595){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(714,1036){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%%
      \put(714,1478){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%%
      \put(714,1919){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%%
      \put(714,2361){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%%
      \put(714,2802){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(816,409){\makebox(0,0){\strut{}$0.75$}}%
      \csname LTb\endcsname%%
      \put(1476,409){\makebox(0,0){\strut{}$0.8$}}%
      \csname LTb\endcsname%%
      \put(2136,409){\makebox(0,0){\strut{}$0.85$}}%
      \csname LTb\endcsname%%
      \put(2795,409){\makebox(0,0){\strut{}$0.9$}}%
      \csname LTb\endcsname%%
      \put(3455,409){\makebox(0,0){\strut{}$0.95$}}%
      \csname LTb\endcsname%%
      \put(4115,409){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig6}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig7.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter{}
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4800.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(525,3118){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(525,3305){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(525,3492){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(525,3679){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(525,3866){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(525,4053){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(651,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(949,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1248,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1546,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1844,2838){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(33,3585){\rotatebox{-270}{\makebox(0,0){\strut{}\tiny{MA order 0 (iid)}}}}%
      \csname LTb\endcsname%%
      \put(1247,4313){\makebox(0,0){\strut{}\tiny{$\tau=3$}}}%
      \csname LTb\endcsname%%
      \put(1437,3563){\makebox(0,0)[r]{\strut{}\tiny{MC}}}%
      \csname LTb\endcsname%%
      \put(1437,3377){\makebox(0,0)[r]{\strut{}\tiny{Ber}}}%
      \csname LTb\endcsname%%
      \put(1437,3191){\makebox(0,0)[r]{\strut{}\tiny{GEV}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(2042,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2340,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2639,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2938,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3236,2838){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2639,4313){\makebox(0,0){\strut{}\tiny{$\tau=4$}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(3435,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3733,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4032,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4330,2838){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4628,2838){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(4031,4313){\makebox(0,0){\strut{}\tiny{$\tau=5$}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(525,1951){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(525,2138){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(525,2325){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(525,2512){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(525,2699){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(525,2886){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(651,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(949,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1248,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1546,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1844,1671){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(33,2418){\rotatebox{-270}{\makebox(0,0){\strut{}\tiny{MA order 32}}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(2042,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2340,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2639,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2938,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3236,1671){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(3435,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3733,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4032,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4330,1671){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4628,1671){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(525,785){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(525,972){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(525,1159){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(525,1346){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(525,1533){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(525,1720){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(651,505){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(949,505){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(1248,505){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(1546,505){\makebox(0,0){\strut{}\tiny{24}}}%
      \csname LTb\endcsname%%
      \put(1844,505){\makebox(0,0){\strut{}\tiny{32}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(33,1252){\rotatebox{-270}{\makebox(0,0){\strut{}\tiny{MA order 64}}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(2042,505){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(2340,505){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(2639,505){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(2938,505){\makebox(0,0){\strut{}\tiny{24}}}%
      \csname LTb\endcsname%%
      \put(3236,505){\makebox(0,0){\strut{}\tiny{32}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(3435,505){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(3733,505){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(4032,505){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(4330,505){\makebox(0,0){\strut{}\tiny{24}}}%
      \csname LTb\endcsname%%
      \put(4628,505){\makebox(0,0){\strut{}\tiny{32}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig7}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig8.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter{}
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4800.00,3600.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(867,595){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(867,1153){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%%
      \put(867,1711){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%%
      \put(867,2269){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%%
      \put(867,2827){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%%
      \put(867,3385){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(969,409){\makebox(0,0){\strut{}$0.75$}}%
      \csname LTb\endcsname%%
      \put(1540,409){\makebox(0,0){\strut{}$0.8$}}%
      \csname LTb\endcsname%%
      \put(2111,409){\makebox(0,0){\strut{}$0.85$}}%
      \csname LTb\endcsname%%
      \put(2682,409){\makebox(0,0){\strut{}$0.9$}}%
      \csname LTb\endcsname%%
      \put(3253,409){\makebox(0,0){\strut{}$0.95$}}%
      \csname LTb\endcsname%%
      \put(3824,409){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(357,2004){\makebox(0,0){\strut{}$r_\text{tr}$}}%
      \csname LTb\endcsname%%
      \put(2396,130){\makebox(0,0){\strut{}$p$-quantile}}%
      \csname LTb\endcsname%%
      \put(1553,3246){\makebox(0,0)[l]{\strut{}\scriptsize{expected}}}%
      \csname LTb\endcsname%%
      \put(4190,2004){\rotatebox{-270}{\makebox(0,0){\strut{}\scriptsize{test statistic value}}}}%
      \csname LTb\endcsname%%
      \put(2968,2775){\makebox(0,0){\strut{}\scriptsize{maximum}}}%
      \csname LTb\endcsname%%
      \put(2968,2513){\makebox(0,0){\strut{}\scriptsize{minimum}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig8}}%
    \gplfronttext
  \end{picture}%
\endgroup

